Taming Fat-Tailed ("Heavier-Tailed'' with Potentially Infinite Variance) Noise in Federated Learning

A key assumption in most existing works on FL algorithms' convergence analysis is that the noise in stochastic first-order information has a finite variance. Although this assumption covers all light-tailed (i.e., sub-exponential) and some heavy-tailed noise distributions (e.g., log-normal, Weibull, and some Pareto distributions), it fails for many fat-tailed noise distributions (i.e., ``heavier-tailed'' with potentially infinite variance) that have been empirically observed in the FL literature. To date, it remains unclear whether one can design convergent algorithms for FL systems that experience fat-tailed noise. This motivates us to fill this gap in this paper by proposing an algorithmic framework called FAT-Clipping (\ul{f}ederated \ul{a}veraging with \ul{t}wo-sided learning rates and \ul{clipping}), which contains two variants: FAT-Clipping per-round (FAT-Clipping-PR) and FAT-Clipping per-iteration (FAT-Clipping-PI). Specifically, for the largest $\alpha \in (1,2]$ such that the fat-tailed noise in FL still has a bounded $\alpha$-moment, we show that both variants achieve $\mathcal{O}((mT)^{\frac{2-\alpha}{\alpha}})$ and $\mathcal{O}((mT)^{\frac{1-\alpha}{3\alpha-2}})$ convergence rates in the strongly-convex and general non-convex settings, respectively, where $m$ and $T$ are the numbers of clients and communication rounds. Moreover, at the expense of more clipping operations compared to FAT-Clipping-PR, FAT-Clipping-PI further enjoys a linear speedup effect with respect to the number of local updates at each client and being lower-bound-matching (i.e., order-optimal). Collectively, our results advance the understanding of designing efficient algorithms for FL systems that exhibit fat-tailed first-order oracle information.

==> Exp_final.tex <==
% !TEX root = ../FedAvg.tex


\section{Appendix II: Experiments} \label{exp}
We provide the full detail of the experiments.
We uses non-i.i.d. versions for MNIST and CIFAR-10, which are described as follows:

\subsection{MNIST}
We study image classification of handwritten digits 0-9 in MNIST and modify the MNIST dataset to a non-i.i.d. version.

To impose statistical heterogeneity, we split the data based on the digits ($p$) they contain in their dataset.
We distribute the data to $m = 100$ workers such that each worker contains only a certain class of digits with the same number of training/test samples.
For example, for $p = 1$, each worker only has training/testing samples with one digit, which causes heterogeneity among different workers.
For $p = 10$, each worker has samples with 10 digits, which is essentially i.i.d. case.
In this way, we can use the digits in worker's local dataset to represent the non-i.i.d. degree qualitatively.
In each communication round, 100 workers run $K$ epochs locally in parallel and then the server samples $n$ workers for aggregation and update.
We make a grid-search experiments for the hyper-parameters as shown in Table ~\ref{tab: 2}.

\begin{table} [!h]
\begin{center}
\caption{Hyper-parameters Tuning.}
\begin{tabular}{c c} 
	\hline
	Server Learning Rate & $\eta \in \{ 1, 10 \}$ \\
	% \hline
	Client Learning Rate & $\eta_L \in \{ 0.001, 0.01, 0.1 \}$ \\
	% \hline
	Local Epochs & $ K \in \{ 1, 5, 10 \}$ \\
	% \hline
	Clients Partition Number & $ n \in \{ 10, 50, 100 \}$ \\
	% \hline
	Non-i.i.d. Degree & $ p \in \{ 1, 2, 5, 10 \}$ \\
	\hline
\end{tabular}
\label{tab: 2}
\end{center}
\end{table}

We run three models: multinomial logistic regression,  fully-connected network with two hidden layers (2NN) (two 200 neurons hidden layers with ReLU followed by an output layer), convolutional neural network (CNN), as shown in Table~\ref{tab: 3}.
The results are shown in Figures~\ref{fig01}, ~\ref{fig2} and ~\ref{fig3}.


\begin{table} [!htb]
\begin{center}
\caption{CNN Architecture for MNIST.}
\begin{tabular}{c c} 
	\hline
	Layer Type & Size \\
	\hline
	Convolution + ReLu & $5 \times 5 \times 32$ \\
	% \hline
	Max Pooling & $2 \times 2$\\
	% \hline
	Convolution + ReLu & $5 \times 5 \times 64$ \\
	% \hline
	Max Pooling & $2 \times 2$\\
	% \hline
	Fully Connected + ReLU & $1024 \times 512$\\
	% \hline
	Fully Connected & $512 \times 10$ \\
	\hline
\end{tabular}
\label{tab: 3}
\end{center}
\end{table}

% \begin{figure*}[!ht]
% 	\begin{minipage}[t]{0.32\linewidth}
% 	\centering
% 	{\includegraphics[width=1.\textwidth]{Figure/fig_1_loss_cnn.pdf}} 
% 	\end{minipage}
% \hspace{0.009\textwidth}
% 	\begin{minipage}[t]{0.32\linewidth}
% 	\centering
% 	{\includegraphics[width=1.\textwidth]{Figure/fig_2_loss_cnn.pdf}}
% 	\end{minipage}
% \hspace{0.009\textwidth}
% 	\begin{minipage}[t]{0.32\linewidth}
% 	\centering
% 	{\includegraphics[width=1.\textwidth]{Figure/fig_3_loss_cnn.pdf}}
% 	\end{minipage}

% 	\begin{minipage}[t]{0.32\linewidth}
% 	\centering
% 	{\includegraphics[width=1.\textwidth]{Figure/fig_1_cnn.pdf}}
% 	\text{(a) Impact of non-i.i.d. datasets.} 
% 	\end{minipage}
% \hspace{0.009\textwidth}
% 	\begin{minipage}[t]{0.32\linewidth}
% 	\centering
% 	{\includegraphics[width=1.\textwidth]{Figure/fig_2_cnn.pdf}}
% 	\text{ {\addtolength{\leftskip}{10 mm}  (b) Impact of worker number.}}
% 	\end{minipage}
% \hspace{0.009\textwidth}
% 	\begin{minipage}[t]{0.32\linewidth}
% 	\centering
% 	{\includegraphics[width=1.\textwidth]{Figure/fig_3_cnn.pdf}}
% 	\text{(c) Impact of local steps}
% 	\end{minipage}
% \caption{Training loss (top) and test accuracy (bottom) for the CNN model with hyper-parameters setting: local learning rate 0.1, global learning rate 1.0: (a) worker number 10, local steps 5 epochs; (b) local steps 5 epochs; (c) 2 digits in each worker's dataset.}
% \label{fig0}
% \end{figure*}%



\begin{figure*}[!htb]
	\begin{minipage}[t]{0.32\linewidth}
	\centering
	{\includegraphics[width=1.\textwidth]{Figure/Appdx/appdx_logistic_loss_acc_worker.pdf}}
	\text{(a) LR}
	\end{minipage}
\hspace{0.009\textwidth}
	\begin{minipage}[t]{0.32\linewidth}
	\centering
	{\includegraphics[width=1.\textwidth]{Figure/Appdx/appdx_2nn_loss_acc_worker.pdf}}
	\text{(b) 2NN}
	\end{minipage}
\hspace{0.009\textwidth}
	\begin{minipage}[t]{0.32\linewidth}
	\centering
	{\includegraphics[width=1.\textwidth]{Figure/Appdx/appdx_cnn_loss_acc_worker.pdf}}
	\text{(c) CNN}
	\end{minipage}
\caption{Training loss (top) and test accuracy (bottom) for three models on MNIST with hyperparameters setting: local learning rate 0.1, global learning rate 1.0, local steps 5 epochs.}
\label{fig01}
\end{figure*}%

\begin{figure*}[!htb]
	\begin{minipage}[t]{0.32\linewidth}
	\centering
	{\includegraphics[width=1.\textwidth]{Figure/Appdx/appdx_logistic_loss_acc_clients100_steps.pdf}}
	\text{(a) LR}
	\end{minipage}
\hspace{0.009\textwidth}
	\begin{minipage}[t]{0.32\linewidth}
	\centering
	{\includegraphics[width=1.\textwidth]{Figure/Appdx/appdx_2nn_loss_acc_clients100_steps.pdf}}
	\text{(b) 2NN}
	\end{minipage}
\hspace{0.009\textwidth}
	\begin{minipage}[t]{0.32\linewidth}
	\centering
	{\includegraphics[width=1.\textwidth]{Figure/Appdx/appdx_cnn_loss_acc_clients100_steps.pdf}}
	\text{(c) CNN}
	\end{minipage}
\caption{Training loss (top) and test accuracy (bottom) for three models on MNIST with hyperparameters setting: local learning rate 0.1, global learning rate 1.0, worker number 100.}
\label{fig2}
\end{figure*}%

\begin{figure*}[t!]
	\begin{minipage}[t]{0.32\linewidth}
	\centering
	{\includegraphics[width=1.\textwidth]{Figure/Appdx/appdx_logistic_loss_acc_clients10_steps.pdf}}
	\text{(a) LR}
	\end{minipage}
\hspace{0.009\textwidth}
	\begin{minipage}[t]{0.32\linewidth}
	\centering
	{\includegraphics[width=1.\textwidth]{Figure/Appdx/appdx_2nn_loss_acc_clients10_steps.pdf}}
	\text{(b) 2NN}
	\end{minipage}
\hspace{0.009\textwidth}
	\begin{minipage}[t]{0.32\linewidth}
	\centering
	{\includegraphics[width=1.\textwidth]{Figure/Appdx/appdx_cnn_loss_acc_clients10_steps.pdf}}
	\text{(c) CNN}
	\end{minipage}
\caption{Training loss (top) and test accuracy (bottom) for three models on MNIST with hyperparameters setting: local learning rate 0.1, global learning rate 1.0, worker number 10.}
\label{fig3}
\end{figure*}%

\subsection{CIFAR-10}
Unless stated otherwise, we use the following default parameter setting: the server learning rate and client learning rate are set to $\eta = 1.0$ and $\eta_L = 0.1$, respectively. 
The local epochs is set to $K=10$.
The total number of clients is set to 100, and the clients partition number is set to $n = 10$.
We use the same strategy to distribute the data over clients as suggested in \cite{mcmahan2016communication}. 
% For the IID setting, we evenly partition all the training data among all clients, i.e., each client observes 600 data;
% for the non-IID setting, we first sort the training data by digit label, then divide all the training data into 200 shards of size 300, and randomly assign 2 shards to each client.
% For the CIFAR-10 dataset, we use the same default parameter setting as MNIST data in Section \ref{MNIST_IID_non_IID}, that is, we let $\eta_g = 1.0$, $\eta_L = 0.1$, $K=10$ and $N = 10$. The total number of clients is set to 100.
For the i.i.d. setting, we evenly partition all the training data among all clients, i.e., each client observes 500 data;
for the non-i.i.d. setting, we first sort the training data by label, then divide all the training data into 200 shards of size 250, and randomly assign two shards to each client.
For the CIFAR-10 dataset, we train our classifier with the ResNet model.
The results are shown in Figure~\ref{fig4} and Figure~\ref{fig5}.

\begin{figure*}[!t]
	\centering
	\begin{subfigure}[b]{0.4\textwidth}
		\includegraphics[width=\textwidth]{Figure/Appdx/iid_num_users_sel_cifar10.pdf}
		\caption{IID.}
	\end{subfigure}
	\hskip1em
	\begin{subfigure}[b]{0.4\textwidth}
		\includegraphics[width=\textwidth]{Figure/Appdx/noniid_num_users_sel_cifar10.pdf}
		\caption{Non-IID.}
	\end{subfigure}
	\caption{Test accuracy with respect to worker number on CIFAR-10 dataset.} 
	\label{fig4}
\end{figure*}

\begin{figure*}[!t]
	\centering
	\begin{subfigure}[b]{0.4\textwidth}
		\includegraphics[width=\textwidth]{Figure/Appdx/iid_local_ep_cifar10.pdf}
		\caption{IID.}
	\end{subfigure}
	\hskip1em
	\begin{subfigure}[b]{0.4\textwidth}
		\includegraphics[width=\textwidth]{Figure/Appdx/noniid_local_ep_cifar10.pdf}
		\caption{Non-IID.}
	\end{subfigure}
	\caption{Test accuracy with respect to different local steps on CIFAR-10 dataset.} 
	\label{fig5}
\end{figure*}




\subsection{Discussion}
\textbf{Impact of non-i.i.d. datasets:}
Figure~\ref{fig01} shows the results of training loss (top) and test accuracy (bottom) for three models under different non-i.i.d. datasets with full and partial worker participation on MNIST.
We can see that the FedAvg algorithm converges under non-i.i.d. datasets with a proper learning rate choice in these cases.
We believe that the major challenge in FL is the non-i.i.d. datasets.
For these datasets with a lower degree of non-i.i.d., the FedAvg algorithm can achieve a good result compared with the i.i.d. case.
For example, when the local dataset in each worker has five digits ($p = 5$) with full (partial) worker participation, the FedAvg algorithm achieves a convergence speed comparable with that of the i.i.d. case ($p = 10$).
This result can be observed in Figure~\ref{fig01} for all three models.
As the degree of non-i.i.d. datasets increases, its negative impact on the convergence is becoming more obvious.
The higher the degree of non-i.i.d., the slower the convergence speed.
As the non-i.i.d. degree increases (from case $p = 10$ to case $p = 1$), it is obvious that the training loss is increasing and test accuracy is decreasing.
For these with high degree of non-i.i.d., the convergence curves oscillate and are highly unstable.
This trend is more obvious for complex models such for CNN in Figure~\ref{fig01}(c).

\textbf{Impact of worker number:}
For full worker participation, the server can have an accurate estimation of the system heterogeneity after receiving the updates for all workers and neutralize this heterogeneity in each communication round.
However, partial worker participation introduces another source of randomness, which leads to zigzagging convergence curves and slower convergence.
In each communication round, the server can only receive a subset of workers based on the sampling strategy.
So the server could only have a coarse estimation of the system heterogeneity and might not be able to neutralize the heterogeneity among different workers for partial worker participation.
This problem is more prominent for highly non-i.i.d. datasets.
It is not unlikely that the digits in these datasets among all active workers are only a proper subset of the total $10$ digits in the original MNIST dataset, especially with highly non-i.i.d. datasets.
For example, for $p = 1$ with $10$ workers in each communication round, it is highly likely that the datasets formed by these ten workers only includes certain small number of digits (say, $4$ or $5$) rather than total $10$ digits.
But for $p = 5$, it is the opposite, that is, the digits in these datasets among these $10$ workers are highly likely to be $10$.
So in each communication round, the server can mitigate system heterogeneity since it covers the training samples with all $10$ digits.
This trend is more obvious for complex models and datasets given the dramatic drop of test accuracy in the result of CIFAR-10 in Figure~\ref{fig4}.

The sample strategy here is random sampling with equal probability without replacement.
In practice, the workers need to be in certain states in order to be able to participate in FL (e.g., in charging or idle states, etc.\cite{eichner2019semi}).
Therefore, care must be taken in sampling and enlisting workers in practice.
We believe that the joint design of sampling schemes, number of workers and the FedAvg algorithm will have a significant impact on the convergence, which needs further investigations.

\textbf{Impact of local steps:}
Figure~\ref{fig2} and Figure~\ref{fig3} shows the results of training loss (top) and test accuracy (bottom) for three models under different local steps with full and partial worker participation respectively.
Figure~\ref{fig5} shows the impact of local steps in CIFAR-10.
One open question of FL is that whether the local steps help the convergence or not.
\citet{li2019convergence} showed a convergence rate $\mathcal{O}(\frac{K}{T})$, i.e., the local steps may hurt the convergence for full and partial worker participation.
In this two figures, we can see that local steps could help the convergence for both full and partial worker participation. 
However, it only has a slight effect on the convergence compared to the effects of non-i.i.d. datasets and number of workers.

\textbf{Comparison with SCAFFOLD:}
We compare SCAFFOLD \citep{karimireddy2019scaffold} with the generalized FedAVg algorithm in this paper in terms of communication rounds, total communication overloads and estimated wall-clock time to achieve certain test accuracy in Table~\ref{tab:addlabel}.
We run the experiments using the same GPU (NVIDIA V100) to ensure the same conditions.
Here, we give a specific comparison for these two algorithms under exact condition.
% The non-i.i.d. dataset is for $digits\_2$ and i.i.d. is for $digits\_10$.
% The learning rate is $\eta_L = 0.1, \eta = 1.0$, and number of local steps $K$ is $5$ epochs.
% We set the target accuracy $\epsilon = 95\%$ for MNIST and $\epsilon = 75\%$ for CIFAR-10.
Note that we divide the total training time to two parts: the computation time when the worker trains the local model and the communication time when information exchanges between the worker and server.
We only compare the computation time and communication time with a fixed bandwidth $20MB/s$ for both uploading and downloading connections.
As shown in Figure~\ref{fig7}, to achieve $\epsilon=75\%$, SCAFFOLD performs less communication round due to the variance reduction techniques.
That is, it spends less time on computation.
However, it needs to communicates as twice as the FedAvg since the control variate to perform variance reduction in each worker needs to update in each round.
In this way, the communication time would be largely prolonged.
% Interestingly, we find that SCAFFOLD is less stable in partial worker participation or large local steps case.
% Note that for variance reduction, the true gradient is needed, which is usually measured by averaging the gradient of all the data samples.
% In order to save the complexity, this true gradient is calculated once for several steps.
% We suppose that in order to get an accurate estimate of the true gradient to perform variance reduction, this true gradient should be synchronized pretty often.
% In partial worker participation or large local steps case, the estimated true gradient is not accurate enough so that unstable convergence occurs.

\begin{figure*}[!ht]
	\centering
	{\includegraphics[width=0.8\textwidth]{Figure/fig_7.pdf}} 
	\caption{Wall-clock time to achieve test accuracy $\epsilon=75\%$ on CIFAR-10 dataset.} 
	\label{fig7}
\end{figure*}


==> Experiments__Haibo_Yang_s_conflicted_copy_2022-10-11_.tex <==
% !TEX root = main.tex

\section{Experiments in Section~\ref{sec:mot}}
In this section, we provide experimental details to demonstrate the fat-tailed noise phenomenon in federated learning. 
We conduct experiments with CNN on CIFAR-10 dataset as shown in Section~\ref{sec:mot}, and provide additional results of logistic regression (LR) model on MNIST and RNN model on Shakespeare dataset. 
% Furthermore, we verify the accuracy of $\alpha$ estimation with logistic regression on MNIST dataset, and this experiment also shows the existence of fat-tailed noise phenomenon.


\subsection{CNN on CIFAR-10 Dataset}

\subsubsection{Experiment details}
% To find the evidences of fat-tailed noise phenomenon in FedAvg, 
We run a convolutional neural network (CNN) model on CIFAR-10 dataset using FedAvg. The CNN architecture is shown in Table~\ref{table:CNN_arch}.
To simulate data heterogeneity across clients, we manually distribute the the data to each client in a label-based partition. 
Specifically, we split the data according to the classes ($p$) of images that each client has. 
Then, we randomly distribute these partitioned data to $m=100$ clients such that each client has only $p$ classes of images in both training and test data, which causes the heterogeneity of data among different clients. 
For example, for $p=10$, each client contains training/test data samples with ten classes.
Since CIFAR-10 has $10$ classes of images, $p=10$ is the nearly i.i.d case. 
For the remaining $p$, each client contains data samples with class $p$. Therefore, the classes ($p$) of images in each client's local dataset can be used to represent the non-i.i.d. degree. 
The smaller the $p$-value, the more heterogeneous the data between clients.

In this experimental setting, we use the global learning rate $\frac{\eta\eta_{L}}{m}=1.0$ and the local learning rate $\eta_{L}=0.1$. 
The batch size is set to 500, and the communication round is $T=4000$.
We run this experiment in different cases, including singleSGD and different local epochs $ \left\{ 1,2,5 \right\}$ and non-iid index $p \in \left\{ 1,2,5,10 \right\}$. Single SGD means one local update step, which is equivalent to mini-batch SGD.

\begin{table}[t!]
\centering
\caption{CNN architecture for CIFAR-10.}
\label{table:CNN_arch}
\begin{tabular}{ll}
\hline
LAYER TYPE             & SIZE     \\ \hline
Convolution + ReLu     & $3\times 32\times 5$   \\
Max Pooling            & $2\times 2$      \\
Convolution + ReLu     & $32\times 64\times 5$  \\
Max Pooling            & $2\times 2$      \\
Fully Connected + ReLU & $1600\times 512$ \\
Fully Connected + ReLU & $512\times 128$  \\
Fully Connected        & $128\times 10$   \\ \hline
\end{tabular}
\end{table}
\FloatBarrier


\subsubsection{Additional experimental results}
We provide additional distributions of the norms of the pseudo-gradient noises in different cases as follows.
From Fig.~\ref{noise_cifar_singleSGD}-~\ref{noise_cifar_localepoch5}, the observation is that the gradient norm statistics are contracted together for more iid cases while dispersed uniformly for more non-iid cases.
This is 

% we can see that the fat-tailed noise exists in both iid and non-iid cases, and when the data is more non-iid, the noise tail is heavier.

\begin{figure*}[htbp]
\centering
\begin{subfigure}[t]{0.24\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{Fig/Add/cifar10_noise_noniid1_localepoch0}
    \caption{$p=1$}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{Fig/Add/cifar10_noise_noniid2_localepoch0}
    \caption{$p=2$}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{Fig/Add/cifar10_noise_noniid5_localepoch0}
    \caption{$p=5$}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{Fig/Add/cifar10_noise_noniid10_localepoch0}
    \caption{$p=10$}
\end{subfigure}
\caption{Distributions of the norms of the pseudo-gradient noises for CIFAR-10 dataset in the case of \textit{Single SGD}.}
\label{noise_cifar_singleSGD}
\vspace{-0.1in}
\end{figure*}


\begin{figure*}[htbp]
\centering
\begin{subfigure}[t]{0.24\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{Fig/Add/cifar10_noise_noniid1_localepoch1}
    \caption{$p=1$}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{Fig/Add/cifar10_noise_noniid2_localepoch1}
    \caption{$p=2$}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{Fig/Add/cifar10_noise_noniid5_localepoch1}
    \caption{$p=5$}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{Fig/Add/cifar10_noise_noniid10_localepoch1}
    \caption{$p=10$}
\end{subfigure}
\caption{Distributions of the norms of the pseudo-gradient noises for CIFAR-10 dataset in the case of \textit{Local Epoch=1}.}
\vspace{-0.1in}
\end{figure*}


\begin{figure*}[htbp]
\centering
\begin{subfigure}[t]{0.24\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{Fig/Add/cifar10_noise_noniid1_localepoch2}
    \caption{$p=1$}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{Fig/Add/cifar10_noise_noniid2_localepoch2}
    \caption{$p=2$}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{Fig/Add/cifar10_noise_noniid5_localepoch2}
    \caption{$p=5$}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{Fig/Add/cifar10_noise_noniid10_localepoch2}
    \caption{$p=10$}
\end{subfigure}
\caption{Distributions of the norms of the pseudo-gradient noises for CIFAR-10 dataset in the case of \textit{Local Epoch=2}.}
\vspace{-0.1in}
\end{figure*}


\begin{figure*}[htbp]
\centering
\begin{subfigure}[t]{0.24\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{Fig/Add/cifar10_noise_noniid1_localepoch5}
    \caption{$p=1$}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{Fig/Add/cifar10_noise_noniid2_localepoch5}
    \caption{$p=2$}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{Fig/Add/cifar10_noise_noniid5_localepoch5}
    \caption{$p=5$}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{Fig/Add/cifar10_noise_noniid10_localepoch5}
    \caption{$p=10$}
\end{subfigure}
\caption{Distributions of the norms of the pseudo-gradient noises for CIFAR-10 dataset in the case of \textit{Local Epoch=5}.}
\label{noise_cifar_localepoch5}
\vspace{-0.1in}
\end{figure*}
\FloatBarrier


\subsection{RNN on Shakespeare Dataset}

\subsubsection{Experiment details}
To provide more evidences of the fat-tailed noise phenomenon, we further run a recurrent neural network (RNN) model on Shakespeare dataset.

Shakespeare dataset is a natural non-iid dataset, and it is built from \textit{The Complete Works of William Shakespeare}~\cite{mcmahan2017communication}. 
The learning task is to predict next character, and there are 80 classes of characters in total.
We use a two-layer LSTM classifier containing 100 hidden units with an 8-dimensional (8D) embedding layer.
The model inputs a sequence of 80 characters, embeds each of the characters into a learned 8D space, and then outputs one character per training sample after two LSTM layers and a densely-connected layer.
The dataset and model are taken from~\cite{li2020federated}.


\subsubsection{Experimental results}
We show the results when local step is set to be one (Single SGD), and multiple local epochs $\{1, 2, 5 \}$. 
In Fig.~\ref{alpha_shakespeare}, we observe that the $\alpha$-value is smaller than 2, and it increases when the number of local epoch increases. This implies that the gradient noise is fat-tailed.
Fig.~\ref{gradient_norm_shakespeare} shows that the distributions of the norms of the pseudo-gradient noises are fat-tailed.


\begin{figure*}[htbp]
\centering
\includegraphics[width=0.5\linewidth]{Fig/Add/shakespeare_alpha}
\caption{Estimation of $\alpha$ for Shakespeare dataset.}
\label{alpha_shakespeare}
\vspace{-0.1in}
\end{figure*}


\begin{figure*}[htbp]
\centering
\begin{subfigure}[t]{0.24\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{Fig/Add/shakespeare_noise_localepoch0}
    \caption{Single SGD}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{Fig/Add/shakespeare_noise_localepoch1}
    \caption{Local Epoch=1}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{Fig/Add/shakespeare_noise_localepoch2}
    \caption{Local Epoch=2}
\end{subfigure}
\begin{subfigure}[t]{0.24\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{Fig/Add/shakespeare_noise_localepoch5}
    \caption{Local Epoch=5}
\end{subfigure}
\caption{Distributions of the norms of the pseudo-gradient noises for Shakespeare dataset.}
\label{gradient_norm_shakespeare}
\vspace{-0.1in}
\end{figure*}



% \subsection{Accuracy of Alpha Estimation (Logistic Regression on MNIST Dataset)}

% \subsubsection{Experiment details}


% \subsubsection{Experimental results}

% \begin{figure*}[htbp]
% \centering
% \includegraphics[width=0.5\linewidth]{Fig/Add/Alpha_compare}
% \caption{Comparisons of accurate $\alpha$ and $\alpha$ approximation on MNIST dataset.}
% \vspace{-0.1in}
% \end{figure*}



\section{Experiments in Section~\ref{sec:numerical}}

In this section, we describe the details of the  numerical experiments from Section~\ref{sec:numerical} and provide some extra experimental results.

\subsection{Experiment details}

\subsubsection{Strongly Convex Model with Synthetic Data}
In these experiments, we consider a strongly convex model for Problem~(\ref{objective}) as follows:
\begin{align*}
    & f_{i}\left( x \right)=\mathbb{E}_{\xi}\left[ f_{i}\left( x,\xi \right) \right]\\
    & f_{i}\left( x,\xi \right)=\frac{1}{2}\left\| x \right\|^{2}+\left\langle \xi,x \right\rangle,
\end{align*}
where $x\in \mathbb{R}^{3\times 1}$ and $\xi$ is a random vector. The optimal solution is $f\left( x^{*} \right)=0$ with $x^{*}=\left[ 0;0;0 \right]$.

To compare the performance of FedAvg, \algpi and \algpr, we consider the noise $\xi$ to be a Cauchy distribution($\alpha<2$, fat-tailed) with a location parameter of $0$ and a scale parameter of $2.1$.

To compare the performance of \algpi and \algpr under different scenarios, we consider the noise $\xi$ having different tail-indexes ($\alpha=0.5, 1.0, \text{ and }1.5$) with the same location parameters of $0$ and the same scale parameters of $1$.

For all the distributions of $\xi$ mentioned above, we use the same experimental setup. There are $m=5$ clients participating in the training. We choose the starting point $x_{0}=\left[ 2;1;1.5 \right]$. We set the global learning rate $\frac{\eta\eta_{L}}{m}=0.1$ and the local learning rate $\eta_{L}=0.1$. The local steps we use is $K=2$, and the communication round is $T=300$. The clipping parameter in \algpi we select is $\lambda=3$, and the clipping parameter in \algpr is $\lambda=5$.

\subsubsection{CNN (Non-convex Model) on the CIFAR-10}
To test the performance of \algpi and \algpr for non-convex function, we run a convolutional neural network (CNN) on CIFAR-10 dataset, which has ten classes of images. We compare \algpi and \algpr with FedAvg under different data heterogeneity. 

To simulate data heterogeneity across clients, we manually distribute the the data to each client in a label-based partition. Specifically, we split the data according to the classes ($p$) of images that each client has. Then, we randomly distribute these partitioned data to $m=10$ clients such that each client has only $p$ classes of images in both training and test data, which causes the heterogeneity of data among different clients. For example, for $p=10$, each client contains training/test data samples with ten classes, and this is the nearly i.i.d case. For the remaining $p$, each client contains data samples with class $p$. Therefore, the classes ($p$) of images in each client's local dataset can be used to represent the non-i.i.d. degree. The smaller the $p$-value, the more heterogeneous the data between clients.

In this experimental setting, we randomly select five clients from $m=10$ clients to participate in each round of the training. We use the global learning rate $\frac{\eta\eta_{L}}{m}=1.0$ and the local learning rate $\eta_{L}=0.1$. The batch size is set to 500. The local epoch we use is two, and the communication round is $T=4000$. The clipping parameter in \algpi we select is $\lambda=50$, and the clipping parameter in \algpr is $\lambda=2$. The architecture of the CNN model is described in Table~\ref{table:CNN_arch}.


\begin{table}[t!]
\centering
\caption{CNN architecture for CIFAR-10.}
\label{table:CNN_arch}
\begin{tabular}{ll}
\hline
LAYER TYPE             & SIZE     \\ \hline
Convolution + ReLu     & $3\times 32\times 5$   \\
Max Pooling            & $2\times 2$      \\
Convolution + ReLu     & $32\times 64\times 5$  \\
Max Pooling            & $2\times 2$      \\
Fully Connected + ReLU & $1600\times 512$ \\
Fully Connected + ReLU & $512\times 128$  \\
Fully Connected        & $128\times 10$   \\ \hline
\end{tabular}
\end{table}

\subsection{Additional experimental Results}
We provide two additional results when applying FedAvg, \algpi and \algpr to the CNN model on CIFAR-10 dataset. In Fig.~\ref{fig:noniid}, we show the percentage of successful training over 5 trials in non-i.i.d. cases when the non-i.i.d. index $p=1$ and $p=5$. These results further support our finding that \alg methods and especially \algpi reduce catastrophic training failures compared to FedAvg.

\begin{figure}[t!]
     \centering
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{noniid1}
         \caption{non-i.i.d. index $p=1$}
         \label{fig:noniid_1}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{noniid5}
         \caption{non-i.i.d. index $p=5$}
         \label{fig:noniid_5}
     \end{subfigure}
        \caption{Percentage of successful training over 5 trials when applying FedAvg, \algpr and \algpi to CIFAR-10 dataset in non-i.i.d. cases.}
        \label{fig:noniid}
\end{figure}


==> Impact/Broader_impact.tex <==
% !TEX root = ../FedAvg.tex

\section*{Broader impact} \label{sec:impact}
Federated learning (FL) is a machine learning setting for many workers collaboratively training a model under a central server.
The algorithm in this paper is not limited to specific models and can be applied to a wide range of applications, including computer vision, natural language processing and many others.
Our paper laid a theoretical foundation for the FL to enjoy the parallelism under non-i.i.d. data as the conventional distributed learning.
This work has the following potential positive impacts on the society:
1) With the unique characteristics of data privacy and communication efficiency, FL is more attractive than conventional distributed learning without obviously slowing down the training;
2) Users of edge devices are more likely to participate in the training of one model given the convenience to join/leave freely.
Users actually can own the data and utilize the extra computation power in their edge device;
This will enable to larger datasets to better train models and in turn a better model to deliver applications with high quality and generate even more data. 

The potential negative consequences include:
1) If the algorithm is used by those with lower levels of domain knowledge, this could increase the risk of failure;
2) Due to the data privacy protection, the dataset in each worker could be adversarial.
This may lead to malicious attacks or non-malicious failures;
3) The sampling process may leads to fairness concerns.
Both non-i.i.d. datasets and partial worker paritcipation introduce extra bias in the overall training.
More research is needed to mitigate the risks, we encourage users to understand the insights behind the algorithms and pay extra attention on the datasets and sampling strategies in practice.
